A statistical formalism for alignment analysis

The detection of anisotropies with respect to a given direction in a vector field is a common problem in astronomy. Several methods have been proposed that rely on the distribution of the acute angles between the data and a reference direction. Different approaches use Monte Carlo methods to quantify the statistical significance of a signal, although often lacking an analytical framework. Here we present two methods to detect and quantify alignment signals and test their statistical robustness. The first method considers the deviance of the relative fraction of vector components in the plane perpendicular to a reference direction with respect to an isotropic distribution. We also derive the statistical properties and stability of the resulting estimator, and therefore does not rely on Monte Carlo simulations to assess its statistical significance. The second method is based on a fit over the residuals of the empirical cumulative distribution function with respect to that expected for a uniform distribution, using a small set of harmonic orthogonal functions, which does not rely on any binning scheme. We compare these methods with others commonly used in the literature, using Monte Carlo simulations, finding that the proposed statistics allow the detection of alignment signals with greater significance.

==> S_random.tex <==
\section{Creating directions with radial symmetry}

% La hipótesis nula ($H_0$) establece que hay simetría esférica en la
% distribución de los vectores $\vec{S}$.
% %
% Para saber la distribución de $\theta$ bajo $H_0$, consideramos que el
% diferencial de área en coordenadas esféricas es (ver Fig.~\ref{F_dA}):
The null hypothesis ($H_0$) establishes that there is sperical symmetry
in the distribution of vectors $\vec{S}$.
%
To know the distribution of $\theta$ under $H_0$, we consider that the
area differential in spherical coordinates is (see Fig.~\ref{F_dA}):

$$
dA = sin(\theta)d\theta d\phi
$$


\begin{figure}
   \centering
\includegraphics[width=0.7\textwidth]{figuras/sphere4.pdf}
   \caption{Area differential in spherical coordinates.}
   \label{F_dA}
\end{figure}      

% Una distribución aleatoria de puntos sobre la esfera, $f_{\Lambda, \Phi}$,
% debe dar como
% resultado un número medio de puntos proporcional al área de un sector
% de la esfera, es decir, si denotamos con 
% $f_{\Theta, \Phi} (\theta, \phi)$ 
% la función de densidad de probabilidad de puntos sobre la superficie
% de una esfera,
A random distribution of points on a sphere, $f_{\Lambda, \Phi}$,
must yield a mean number of points proportional to the area of a section
of the sphere, i.e., if we name the probability density function of points
on the surface of a sphere $f_{\Theta, \Phi} (\theta, \phi)$,
$
$$
dN = \int_{dA} f_{\Theta, \Phi} (\theta, \phi).
$$
$
If $f_{\Theta, \Phi} (\theta, \phi)$ is uniform, then
%
$$
dN \propto dA,
$$



% Se utiliza la convención de denotar con letras mayúsculas (e.g. $\Theta$, $\Lambda$, $\Phi$) las variables aleatorias (V.A.) y con letras
% minúsculas (e.g. $\theta$, $\lambda$, $\phi$) los valores de las V.A.
We employ the convention of naming with upper--case characters (e.g. $\Theta$, $\Lambda$, $\Phi$) the random variables (R.V.) and with lower--case characters (e.g. $\theta$, $\lambda$, $\phi$) the values of said R.V.

% De manera similar, se puede trabajar con el hemisferio superior de la
% esfera en función de las consideraciones de simetría, con lo cual
% planteamos la distribución para $\Lambda$ y $\Phi$:
In a similar fashion, one can work with the upper hemisphere of the sphere 
by way of the symmetry considerations, with which we propose the distribution for
$\Lambda$ y $\Phi$:

$$
dN = \int_{dA} f_{\Lambda, \Phi} \propto dA
$$


% Las dos variables son separables, o sea que $f_{\Lambda, \Phi}(\lambda,
% \phi)=f_{\Lambda}(\lambda)f_{\Phi}(\phi)$. Por simetría,
The two variables are separable, meaning $f_{\Lambda, \Phi}(\lambda,
\phi)=f_{\Lambda}(\lambda)f_{\Phi}(\phi)$. Given the symmetry, 
%
$$
f_{\Phi}(\phi) = U(0, 2\pi)
$$
%
% donde $U(a, b)$ es la distribución uniforme entre $a$ y $b$.  Para la
% distribución de $\Lambda$ vemos que el número de puntos $dN$ en una
% franja entre $\lambda$ y $\lambda+d\lambda$ debe ser proporcional al área
% de esa franja, es decir,
where $U(a, b)$ is the uniform distribution between $a$ and $b$.
For the distribution of $\Lambda$ we see that the number of points $dN$ in a strip
between $\lambda$ and $\lambda+d\lambda$ must be proportional to the area of said strip,
i.e.,

$$
dN \sim \sin(\lambda)d\lambda
$$

Keeping in mind that
%
$$
\int_0^{\pi/2} \sin(\lambda)d\lambda = -\cos(\lambda)
\Bigg|_{0}^{\pi/2} = 1,
$$
%
we can then build the probability distribution function
$f_{\Lambda}(\lambda)$:
%
\[   
f_{\Lambda}(\lambda) = 
\begin{cases}     
\sin(\lambda) & \qquad \lambda \in [0, \pi/2] \\
0 &\qquad c.c.,
\end{cases}
\]
%
where we can verify that
%
$$
\int_{-\infty}^{\infty}  f_{\Lambda}(\lambda) d\lambda =
\int_0^{\pi/2} \sin(t)dt = 1.
$$


Then, the probability function $F_{\Lambda}(\lambda)$ is:
%
$$
F_{\Lambda}(\lambda) = \int_0^{\lambda} \sin(t)dt =
1-\cos(\lambda)
$$
%
which is an increasing function ranging from $(0, 0)$ to $(\pi/2, 1)$ (see
Fig.~\ref{F_flambda}).
%
To generate a random variable with distribution
%Para generar una variable aleatoria con distribución
$f_{\Lambda}(\lambda)$ one can use the method of the inverse function.
%
To that effect we look for the inverse of $F_{\Lambda}(\lambda)$:
%Para ello buscamos la inversa de $F_{\Lambda}(\lambda)$:
%
$$
u = 1-\cos(\lambda) \implies \lambda=acos(1-u)
$$
%
% para una variable uniforme estándar $u \sim U(0, 1)$. Luego,
% como la distribución de $1-u$ es la misma que la
% distribución de $u$,
for a standard uniform variable $u \sim U(0, 1)$. Then,
given that the distribution of $1-u$ is the same as that of $u$,

\begin{equation}
\lambda = acos(u), \qquad 0<u<1
\end{equation}


\begin{figure}
   \centering
   \includegraphics[width=0.7\textwidth]{figuras/F.pdf}
   \caption{Distribution of $\lambda$, $F_{\Lambda}(\Lambda)=1-cos(\lambda)$.}
   \label{F_flambda}
\end{figure}      
 

In a similar fashion,
%De manera similar, 

\[   
f_{\Theta}(\theta) = 
\begin{cases}     
   \frac{1}{2}\sin(\theta) & \qquad \theta \in [0, \pi] \\
0 &\qquad c.c.
\end{cases}
\]

%ya que 
given that

$$
\int_{-\infty}^{\infty}  f_{\Theta}(\theta) d\theta = \int_0^{\pi} \sin(t)dt = 2
$$


%La función de probabilidad $F_{\Theta}(\theta)$ es entonces:
Then, the probability fucntion $F_{\Theta}(\theta)$ is:

$$
F_{\Theta}(\theta) = \int_0^{\theta} \sin(t)dt =
\frac{1}{2}-\frac{1}{2}\cos(\theta)
$$
 
%por lo que:
and so:

\begin{equation}
\theta = acos(1-2u), \qquad 0<u<1 \implies -1<1-2u<1
\end{equation}


%Finalmente, 
Finally,

\begin{equation}
   \beta = \tan(\lambda) = \tan(acos(u)), \qquad u \sim U(0, 1)
\end{equation}

% Esta última expresión permite generar una muestra aleatoria de $\beta$ a
% partir de una muestra aleatoria de $u$.
% %
% El código de python para generar una muestra aleatoria de $\beta$
% puede ser:
% %
The last expression allows for the generation of a random sample of $\beta$
from a random sample of $u$.
%
The python code for generating a random sample of $\beta$ might be:
%
\begin{minted}[escapeinside=||, bgcolor=whitesmoke, fontsize=\small]{python}
def f1(N):
    u = np.random.uniform(0, 1, N)
    b = np.tan(np.arccos(u))
    return b
\end{minted}


\subsection{method 2: accept reject}

% Otro método consiste en generar puntos dentro de una esfera,
% eliminando por un método de "fuerza bruta" los puntos que no están
% dentro de la esfera, y luego normalizar:
% %
Another method consists of generating points inside a sphere \textcolor{red}{(no será "cubo" acá?)},
eliminating by "brute force" those that are not inside the sphere, and
then normalizing;
%
\begin{minted}[escapeinside=||, bgcolor=whitesmoke, fontsize=\small]{python}
def f2(N):
    X = np.random.uniform(0, 1, (3*N, 3))
    n =  np.linalg.norm(X, axis=1)
    filtro = n<1
    s_par = X[filtro][:,2]
    s_perp = np.linalg.norm(X[filtro][:,0:2], axis=1) 
    b = s_perp / s_par
    return b
\end{minted}
 



\subsection{Method 3: using normal R.V.}

% Otro método consiste en generar V.A. normales (estándar), lo que se
% puede hacer de manera eficiente con el método de Box-Müller
% \citep{golder_boxmuller_1976}. Este método evita la acumulación de
% puntos en lo que serían las esquinas del cubo del método anterior,
% debido a la disminución de la probabilidad de tener puntos lejos del
% centro.

Another method consists of generating normal (standard) R.V., which
can be done in an efficient manner with the Box-Müller method
\citep{golder_boxmuller_1976}. This method avoids the accumulation of points
in what would be the corners of the cube in the previous method given the 
lower probability of having points far from the center.

% La justificación de este método radica en la propiedad reproductiva de
% la función normal. En efecto, si se tienen 3 V.A. independientes X, Y y Z con
% distribución normal,
The justification of this method lies in the reproductive property of the 
normal function. Indeed, if one has 3 independent R.V., X, Y, and Z, 
with normal distribution,

$$
f(x) = \frac{1}{\sqrt{2\pi}}exp(-1/2 x^2)
$$

% y similarmente para $y$, $z$. Luego, de la distribución conjunta para
% $v=(x, y, z)$:
and similarly for $y$, $z$. Then, from the joint distribution for
$v=(x, y, z)$:

\begin{align*}
   f(x, y, z) &= \frac{1}{\sqrt{2\pi}}exp\left(-\frac{x^2}{2}\right) 
                  \frac{1}{\sqrt{2\pi}}exp\left(-\frac{y^2}{2}\right) 
                  \frac{1}{\sqrt{2\pi}}exp\left(-\frac{z^2}{2}\right) \\
   &= \frac{1}{(2\pi)^{3/2}} exp\left(-\frac{1}{2} |\vec{v}|^2\right)\\
\end{align*} 
%
% \noindent
% donde $|\vec{v}|$ es la norma euclídea de $\vec{v}$. Se sigue entonces
% que la distribución depende de la distancia al centro y no de la
% orientación, y por lo tanto los vectores $\vec{v}/|\vec{v}|$, que
% tienen norma igual a 1, están orientados en
% direcciones aleatorias.
\noindent
where $|\vec{v}|$ is the euclidean norm of $\vec{v}$. It follows then that
the distribution depends on the distance to the center and not on
the orientation, and so the vectors $\vec{v}/|\vec{v}|$, that
have unit norm, are oriented in random directions.
%
\begin{minted}[escapeinside=||, bgcolor=whitesmoke, fontsize=\small]{python}

def f3(N):
    X = np.random.normal(loc=0, scale=1, size=(N, 3))
    n =  np.linalg.norm(X, axis=1)
    s_par = X[:,2]
    s_perp = np.linalg.norm(X[:,0:2], axis=1) 
    b = s_perp / s_par
    return b
\end{minted}
 
% A manera de verificación, podemos comparar los histogramas de muestras
% aleatorias de $\beta$ con los 3 métodos (Fig.~\ref{F_3metodos}).
As verification, we can compare the histograms of the random samples
of $\beta$ with the 3 methods (Fig.~\ref{F_3metodos}).
%
% Cabe mencionar que existen otros métodos \citep{cook_rational_1957, marsaglia_choosing_1972}
It is noteworthy to mention that there are other methods \citep{cook_rational_1957, marsaglia_choosing_1972}

\begin{figure}
   \centering
   \includegraphics[width=0.7\textwidth]{figuras/beta_rvs.pdf}
%   \caption{Histogramas de muestras aleatorias de la variable
%   $\beta$ obtenidos con 3 métodos diferentes.}
   \caption{Histograms of different random samples of the variable
   $\beta$ obtained with 3 different methods.}
   \label{F_3metodos}
\end{figure}     

